A GDPR-compliant Risk Management Approach based on Threat Modelling and ISO 27005

Computer systems process, store and transfer sensitive information which makes them a valuable asset. Despite the existence of standards such as ISO 27005 for managing information risk, cyber threats are increasing, exposing such systems to security breaches, and at the same time, compromising users' privacy. However, threat modelling has also emerged as an alternative to identify and analyze them, reducing the attack landscape by discarding low-risk attack vectors, and mitigating high-risk ones. In this work, we introduce a novel threat-modelling-based approach for risk management, using ISO 27005 as a baseline for integrating ISO 27001/27002 security controls with privacy regulations outlined in the European General Data Protection Regulation (GDPR). In our proposal, risk estimation and mitigation is enhanced by combining STRIDE and attack trees as a threat modelling strategy. Our approach is applied to an IoT case study, where different attacks are analyzed to determine their risk levels and potential countermeasures.

==> sections/method.tex <==
This research follows the design science methodology [27t], the activities of there are developed in 3 phases: 

\begin{enumerate}[label=(\roman*)]
	\item \textit{Scope and objectives:} This phase consists on defining the problem, and discovering goals to define objectives. Here a systematic literature search for reports on cyber attacks was made to define an scenario for identifying a threat catalogue, and defining attacker profiles.
	\item \textit{Design and development:} The risk approach given by the ISO 27005 standard is used as a baseline for threat modelling and risk management. Here, qualitative and quantitative methods are employed to develop risk matrices for our previous threat catalogue. The aim is to use these matrices as inputs for modelling attack and defense trees for risk management.
	\item \textit{Evaluation and Analysis: } The final phase involves evaluating the proposed risk assessment approach, and presenting results. Once the qualitative and quantitative analysis of potential attack vectors has been carried out, security controls based on ISO 27001/27002 are proposed along with additional privacy controls based on GDPR. Finally, inherent and residual risk levels are analysed before and after applying these controls, respectively.
\end{enumerate}

It is important to highlight that in our proposal, risk management is driven by threat modelling, using STRIDE for threat identification, and both attack and defense trees for determining inherent and residual risk levels. For the application of STRIDE, \textit{Microsoft Threat Modelling Tool} is used to identify threats [4][5][6] within the scenario defined in \textit{Phase (i)}. Conversely, \textit{Attack-Defense Tree Tool (ADTool)} is used during the creation of attack and defense trees [7]. This tool allows modelling scenarios for identifying attack vectors. In addition, ADTool allows performing quantitative analysis on the tree nodes to identify attack costs, attacker skill levels, time to deploy countermeasures, etc. In the next section, the proposed risk management approach is explained in detail.
